Towards Real Time Compton Imaging in Demanding Conditions

Compton cameras are radiation detectors that provide spatial information on the origin of the {\gamma}-ray sources based on the Compton scattering effect. Many applications require these detectors to be used at high counting rate. As such, the preprocessing of the detections as well as the imaging algorithms are required to be time-efficient in order for the data to be processed in real time. In this work, optimizations to the preprocessing of events in Compton cameras based on monolithic crystals, with special focus on event identification, were implemented using a parallelizable algorithm. Regarding imaging, an established 3D back projection algorithm was parallelized and implemented using SYCL. The parallel implementation of the algorithm was included without and with several optimizations such as the pre-computing values, discarding low impact contributions based on angle, and selecting an efficient shape of the image universe. The implementations were tested with Intel CPUs, GPUs, and NVIDIA GPUs. An outlook into the study of algorithms to reconstruct the position of interaction within Compton cameras based on monolithic crystals into segmented regions and other next steps is included.

==> camera.tex <==
\begin{tikzpicture}[scale=0.19, every node/.style={transform shape}]

    \tikzcuboid{%
        shiftx=10cm,%
        shifty=-4cm,%
        %shiftz=-4cm,%
        scale=1.00,%
        rotation=90,%
        densityx=0,%
        densityy=0,%
        densityz=0,%
        dimx=16,%
        dimy=3,%
        dimz=16,%
        linefront=green!75!black,%
        linetop=green!50!black,%
        lineright=green!25!black,%
        fillfront=green!25!white,%
        filltop=green!50!white,%
        fillright=green!75!white%
    };

    \draw[vector1] (-1.7,.45) -- (9.5,.8);
    \draw[vector1] (-0.25,4.15) -- (9.8,4.55);
    \draw[vector1] (1.25,1.25) -- (12.5,.5);

    \tikzcuboid{%
        shiftx=0cm,%
        shifty=0cm,%
        scale=1.00,%
        rotation=90,%
        densityx=0,%
        densityy=0,%
        densityz=0,%
        dimx=8,%
        dimy=2,%
        dimz=8,%
        linefront=blue!75!black,%
        linetop=blue!50!black,%
        lineright=blue!25!black,%
        fillfront=blue!25!white,%
        filltop=blue!50!white,%
        fillright=blue!75!white%
    }

    \def\Ra{13}
    \coordinate (O1) at (1.25,1.25);
    \coordinate (J1) at (170:\Ra); 
    \jetcone{O1}{J1}{1.2}{0.2}
    \def\Rb{14}
    \coordinate (O2) at (-0.25,4.15);
    \coordinate (J2) at (165:\Rb); 
    \jetcone{O2}{J2}{2.2}{0.8}
    \def\Rc{14}
    \coordinate (O3) at (-1.7,.45);
    \coordinate (J3) at (180:\Rb); 
    \jetcone{O3}{J3}{2.2}{.8}
    %\node[thick, text=red] at (-12,1.7) {\textbullet};
    \node at (-12.28,1.48)  [red, circle,fill,inner sep=4.5pt]{};

    \node[thick] at (-1,9.5) {\Huge \textbf{Scatterer}};

    \node[thick] at (8,13.5) {\Huge \textbf{Absorber}};
    

\end{tikzpicture}

==> crystal.tex <==
\begin{tikzpicture}[scale=0.6, every node/.style={transform shape}]

        \draw[thick] (0,0) -- (5,0) -- (5,3) -- (0,3) -- (0,0);
        \draw[thick] (0,0) -- (0,-.25) -- (5,-.25) -- (5,0);
        \foreach \Pointt in {1, 2, 3, 4}{
            \draw (\Pointt,3) -- (\Pointt,-.25);
        }
        \draw[->, decorate,decoration={coil,aspect=0}] (4,3.5) -- (2.25,2.25);
        \draw[orange] (2,1.75) -- (2.25,2.25) -- (3,.75);
        \node[text=red] at (2.5,1.5) {\textbullet};

        \draw[thick] (6,0) -- (11,0) -- (11,3) -- (6,3) -- (6,0);
        \draw[thick] (6,0) -- (6,-.25) -- (11,-.25) -- (11,0);
        \foreach \Pointt in {1, 2, 3, 4}{
            \draw ({\the\numexpr (\Pointt + 6) },0) -- ({\the\numexpr (\Pointt + 6) },-.25);
        }
        \draw[->, decorate,decoration={coil,aspect=0}] (10,3.5) -- (8.25,2.25);
        \draw[orange] (7.125,0) -- (8.25,2.25) -- (9.375,0);
        \node[text=red] at (8.25,2.25) {\textbullet};

        \draw[thick] (12,0) -- (17,0) -- (17,3) -- (12,3) -- (12,0);
        \draw[thick] (12,0) -- (12,-.25) -- (17,-.25) -- (17,0);
        \foreach \Pointt in {1, 2, 3, 4}{
            \draw ({\the\numexpr (\Pointt + 12) },0) -- ({\the\numexpr (\Pointt + 12) },-.25);
        }
        \foreach \Pointt in {.625, 1.25, 1.875, 2.5, 3.125, 3.75, 4.375}{
            \draw[dashed] ({\the\numexpr (\Pointt + 12) },0) -- ({\the\numexpr (\Pointt + 12) },3);
        }
        \draw[dashed] (12,1) -- (17,1);
        \draw[dashed] (12,2) -- (17,2);
        \draw[->, decorate,decoration={coil,aspect=0}] (16,3.5) -- (14.25,2.25);
        \draw[orange] (13.125,0) -- (14.25,2.25) -- (15.375,0);
        \node[text=red] at (14.1875,2.5) {\textbullet};

    \end{tikzpicture}

==> expected.tex <==
\begin{tikzpicture}[scale=0.675, every node/.style={transform shape}]

            \draw[->] (0,0) -> (12,0);

            \foreach \Pointn in {.5, 1.5, 3.5, 4.9, 7.3, 8.7, 9.8, 11.3}{
                \node[text=gray] at (\Pointn,.1) {\textbullet};
            };

            \foreach \Pointx in {0, .2, .5, .6, .7}{
                \foreach \Pointt/\Pointy in {1/.3, 3.2/.5, 3.7/.7, 6/.9, 9/1.1}{
                    \node[text=gray] at ({\the\numexpr (\Pointt + \Pointx) },\Pointy) {\textbullet};
                };
            };
        \end{tikzpicture}

        \begin{tikzpicture}[scale=0.7, every node/.style={transform shape}]

            \draw[->] (0,0) -> (12,0);

            \foreach \Pointn in {.5, 1.5, 3.5, 4.9, 7.3, 8.7, 9.8, 11.3}{
                \node at (\Pointn,.1) {\textbullet};
            };

            \foreach \Pointx in {0, .2, .5, .6, .7}{
                \foreach \Pointt/\Pointy/\Pointc in {1/.3/blue, 3.2/.5/red, 3.7/.7/green, 6/.9/magenta, 9/1.1/orange}{
                    \node[text=\Pointc] at ({\the\numexpr (\Pointt + \Pointx) },\Pointy) {\textbullet};
                };
            };

        \end{tikzpicture}
        
        \begin{tikzpicture}[scale=0.7, every node/.style={transform shape}]
            \draw[->] (0,0) -> (12,0);

            \foreach \Pointn in {.5, 1.5, 3.5, 4.9, 7.3, 8.7, 9.8, 11.3}{
                \node at (\Pointn,.1) {\textbullet};
            };

            \draw (0.9,.2) -> (1.8,.2);
            \draw (3.1,.4) -> (4.0,.4);
            \draw (4.1,.6) -> (5.0,.6);
            \draw (5.9,.8) -> (6.8,.8);
            \draw (8.6,1.) -> (9.5,1.);

            \foreach \Pointx in {0, .2, .5, .6, .7}{
                \foreach \Pointt/\Pointy/\Pointc in {1/.3/blue, 3.2/.5/red, 3.7/.7/green, 6/.9/magenta, 9/1.1/orange}{
                    \node[text=\Pointc] at ({\the\numexpr (\Pointt + \Pointx) },\Pointy) {\textbullet};
                };
            };

            \node[text=blue] at (1.5,.1) {\textbullet};
            \node[text=red] at (3.5,.1) {\textbullet};
            \node[text=orange] at (8.7,.1) {\textbullet};
            \node[text=green] at (4.9,.1) {\textbullet};
            \node[text=red] at (3.7,.7) {\textbullet};
            \node[text=red] at (3.9,.7) {\textbullet};

            \node[text=black] at (9.6,1.1) {\textbullet};
            \node[text=black] at (9.7,1.1) {\textbullet};

        \end{tikzpicture}
        
        \begin{tikzpicture}[scale=0.7, every node/.style={transform shape}]
    
            \draw[->] (0,0) -> (12,0);

            \foreach \Pointn in {.5, 1.5, 3.5, 4.9, 7.3, 8.7, 9.8, 11.3}{
                \node at (\Pointn,.1) {\textbullet};
            };

            \node[text=blue] at (1.5,.1) {\textbullet};
            \node[text=red] at (3.5,.1) {\textbullet};
            \node[text=orange] at (8.7,.1) {\textbullet};
            \node[text=orange] at (9.8,.1) {\textbullet};

            \draw (0.9,.2) -> (1.8,.2);
            \draw (3.1,.4) -> (4.5,.4);
            \draw (5.9,.8) -> (6.8,.8);
            \draw (8.6,1.) -> (9.9,1.);

            \foreach \Pointx in {0, .2, .5, .6, .7}{
            \foreach \Pointt/\Pointy/\Pointc in {1/.3/blue, 3.2/.5/red, 3.7/.7/red, 6/.9/magenta, 9/1.1/orange}{
                    \node[text=\Pointc] at ({\the\numexpr (\Pointt + \Pointx) },\Pointy) {\textbullet};
                };
            };

        \end{tikzpicture}
